SAMPart3D: Segment Any Part in 3D Objects

3D part segmentation is a crucial and challenging task in 3D perception, playing a vital role in applications such as robotics, 3D generation, and 3D editing. Recent methods harness the powerful Vision Language Models (VLMs) for 2D-to-3D knowledge distillation, achieving zero-shot 3D part segmentation. However, these methods are limited by their reliance on text prompts, which restricts the scalability to large-scale unlabeled datasets and the flexibility in handling part ambiguities. In this work, we introduce SAMPart3D, a scalable zero-shot 3D part segmentation framework that segments any 3D object into semantic parts at multiple granularities, without requiring predefined part label sets as text prompts. For scalability, we use text-agnostic vision foundation models to distill a 3D feature extraction backbone, allowing scaling to large unlabeled 3D datasets to learn rich 3D priors. For flexibility, we distill scale-conditioned part-aware 3D features for 3D part segmentation at multiple granularities. Once the segmented parts are obtained from the scale-conditioned part-aware 3D features, we use VLMs to assign semantic labels to each part based on the multi-view renderings. Compared to previous methods, our SAMPart3D can scale to the recent large-scale 3D object dataset Objaverse and handle complex, non-ordinary objects. Additionally, we contribute a new 3D part segmentation benchmark to address the lack of diversity and complexity of objects and parts in existing benchmarks. Experiments show that our SAMPart3D significantly outperforms existing zero-shot 3D part segmentation methods, and can facilitate various applications such as part-level editing and interactive segmentation.

==> table/partnete.tex <==
\begin{table}[!ht]
\centering

\resizebox{0.3\textwidth}{!}{

\begin{tabular}{c|c}
\hline
 Method  & Overall (miou) \\
 \hline 

 PointCLIPv2 &   16.1  \\

 PartSLIP   &  34.4  \\ 
                      
 ZeroPS     &     39.3  \\ 

 PartDistill   &  39.9  \\ 
  
 Ours  & \textbf{41.2} \\ \hline
\end{tabular}
}
\vspace{-5pt}
\caption{Zero-shot semantic segmentation on PartNetE, reported in mIoU (\%). 
}
\vspace{-5pt}
\label{tab:sem_partnete}
\end{table}
